Real Time Scheduling Framework for Multi Object Detection via Spiking Neural Networks

Given the energy constraints in autonomous mobile agents (AMAs), such as unmanned vehicles, spiking neural networks (SNNs) are increasingly favored as a more efficient alternative to traditional artificial neural networks. AMAs employ multi-object detection (MOD) from multiple cameras to identify nearby objects while ensuring two essential objectives, (R1) timing guarantee and (R2) high accuracy for safety. In this paper, we propose RT-SNN, the first system design, aiming at achieving R1 and R2 in SNN-based MOD systems on AMAs. Leveraging the characteristic that SNNs gather feature data of input image termed as membrane potential, through iterative computation over multiple timesteps, RT-SNN provides multiple execution options with adjustable timesteps and a novel method for reusing membrane potential to support R1. Then, it captures how these execution strategies influence R2 by introducing a novel notion of mean absolute error and membrane confidence. Further, RT-SNN develops a new scheduling framework consisting of offline schedulability analysis for R1 and a run-time scheduling algorithm for R2 using the notion of membrane confidence. We deployed RT-SNN to Spiking-YOLO, the SNN-based MOD model derived from ANN-to-SNN conversion, and our experimental evaluation confirms its effectiveness in meeting the R1 and R2 requirements while providing significant energy efficiency.

==> 07related_work.tex <==
\section{Related Work}
\label{sec:related_work}


ANNs have been extensively researched for their high accuracy in object detection tasks, but their significant energy consumption limits their suitability for embedded environments with constrained battery and computing resources.
Addressing this, recent developments have pivoted towards SNN-based detection models that offer comparable accuracy to ANNs but with substantially reduced energy consumption.
Spiking-YOLO~\cite{KPN20}, a pioneering model in this space, leverages an ANN-to-SNN conversion method to transform the YOLOv3~\cite{RJF18} into an SNN, achieving similar detection accuracy to its ANN counterpart while consuming about 280 times less energy.
Similarly, EMS-YOLO~\cite{SCH23} advances the field by directly training an SNN to operate efficiently with fewer timesteps (e.g., four), maintaining high detection accuracy and further enhancing energy efficiency.
These innovations mark a significant step towards integrating advanced neural network technologies in energy-constrained embedded systems, highlighting the potential of SNNs as a sustainable alternative to traditional ANNs for object detection and beyond.



SNNs perform inference using binary spikes, requiring a substantial number of timesteps to achieve high accuracy.
However, as the number of necessary timesteps increases, both execution time and energy consumption rise linearly.
Recent research has focused on achieving comparable or higher accuracy with fewer timesteps to address this issue.
DT-SNN~\cite{LMG23} utilizes entropy to measure the reliability of information extracted by SNNs, reducing timesteps during inference without compromising accuracy.
TopSpark~\cite{PRVS23} proposes an adaptive methodology to decrease timesteps in training and inference phases according to changing environments.
These studies primarily target the image classification task and aim to minimize timesteps, not ensuring timely execution for each object detection task.
Conversely, \sys{} specifically targets the MOD tasks, dynamically adjusting timesteps to guarantee timely execution for all tasks, \hb{as MOD presents more challenges and complexities than standard classification problems}.

